Computational Modelling of Plurality and Definiteness in Chinese Noun Phrases

Theoretical linguists have suggested that some languages (e.g., Chinese and Japanese) are "cooler" than other languages based on the observation that the intended meaning of phrases in these languages depends more on their contexts. As a result, many expressions in these languages are shortened, and their meaning is inferred from the context. In this paper, we focus on the omission of the plurality and definiteness markers in Chinese noun phrases (NPs) to investigate the predictability of their intended meaning given the contexts. To this end, we built a corpus of Chinese NPs, each of which is accompanied by its corresponding context, and by labels indicating its singularity/plurality and definiteness/indefiniteness. We carried out corpus assessments and analyses. The results suggest that Chinese speakers indeed drop plurality and definiteness markers very frequently. Building on the corpus, we train a bank of computational models using both classic machine learning models and state-of-the-art pre-trained language models to predict the plurality and definiteness of each NP. We report on the performance of these models and analyse their behaviours.

==> results/ModelsExperimentResults.tex <==
\usepackage{booktabs}
\usepackage{multirow}
\usepackage[figuresright]{rotating}

\begin{document}

% \begin{table}[H]
% \caption{The results of algorithms performance for plurality}
% \label{plurality model performance}
% \centering
% \small
% \begin{tabular}{lccccccccccccc}
% \hline
%   & \multicolumn{3}{c}{{\textsc{Single}}} & \multicolumn{3}{c}{{\textsc{Plurality}}} & \multicolumn{3}{c}{{\textsc{Macro avg}}} & \multicolumn{3}{c}{{\textsc{Weighted avg}}} &\\
%   & P & R & F & P & R & F & P & R & F & P & R & F & Acc.\\
%   \hline
%   RF & 7954 & 9886 & 8815 & 8263 & 1751 & 2890 & 8108 & 5819 & 5853 & 8026 & 7969 & 7419 & 7969\\
%   LR & 8371 & 9423 & 8866 & 6844 & 4055 & 5092 & 7608 & 6739 & 6979 & 8011 & 8158 & 7977 & 8158\\
%   SVM & 8373 & 9391 & 8853 & 6739 & 4083 & 5085 & 7556 & 6737 & 6969 & 7988 & 8140 & 7965 & 8140\\
%   LSTM & 8532 & 9470 & 8977 & 7330 & 4718 & 5741 & 7931 & 7094 & 7359 & 8249 & 8350 & 8214 & 8350\\
%   BERT (base) & 8910 & 9266 & 9084 & 7265 & 6326 & 6763 & 8088 & 7796 & 7924 & 8523 & 8573 & 8537 & 8573\\
%   BERT (wwm,base) & 8933 & 9252 & 9089 & 7256 & 6416 & 6810 & 8094 & 7834 & 7950 & 8538 & 8583 & 8552 & 8583\\
%   BERT (multilingual,base) & 8861 & 9245 & 9049 & 7152 & 6146 & 6611 & 8007 & 7696 & 7830 & 8458 & 8515 & 8474 & 8515\\
%   RoBERTa (base) & 8880 & 9316 & 9093 & 7363 & 6191 & 6726 & 8121 & 7753 & 7909 & 8522 & 8579 & 8535 & 8579\\
%   RoBERTa (large) & 8864 & 9365 & 9108 & 7480 & 6109 & 6725 & 8172 & 7737 & 7917 & 8538 & 8598 & 8546 & 8598\\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[H]
% \caption{The results of algorithms performance for definiteness}
% \label{definiteness model performance}
% \centering
% \small
% \begin{tabular}{lccccccccccccc}
% \hline
%   & \multicolumn{3}{c}{{\textsc{Undefiniteness}}} & \multicolumn{3}{c}{{\textsc{Definitness}}} & \multicolumn{3}{c}{{\textsc{Macro avg}}} & \multicolumn{3}{c}{{\textsc{Weighted avg}}} &\\
%   & P & R & F & P & R & F & P & R & F & P & R & F & Acc.\\
%   \hline
%   RF & 6669 & 8014 & 7280 & 7058 & 5434 & 6140 & 6863 & 6724 & 6710 & 6851 & 6809 & 6747 & 6809\\
%   LR & 7246 & 7600 & 7419 & 7101 & 6705 & 6897 & 7173 & 7153 & 7158 & 7178 & 7182 & 7175 & 7182\\
%   SVM & 7173 & 7643 & 7401 & 7095 & 6565 & 6820 & 7134 & 7104 & 7110 & 7137 & 7140 & 7129 & 7140\\
%   LSTM & 7942 & 7633 & 7784 & 7415 & 7744 & 7575 & 7678 & 7688 & 7680 & 7695 & 7684 & 7687 & 7684\\
%   BERT (base) & 8334 & 8203 & 8268 & 7986 & 8130 & 8057 & 8160 & 8166 & 8163 & 8171 & 8169 & 8169 & 8169\\
%   BERT (wwm, base) & 8230 & 8433 & 8330 & 8161 & 7931 & 8044 & 8195 & 8182 & 8187 & 8198 & 8198 & 8197 & 8198\\
%   BERT (multilingual, base) & 8041 & 8424 & 8228 & 8099 & 7659 & 7873 & 8070 & 8041 & 8050 & 8068 & 8066 & 8062 & 8066\\
%   RoBERTa (base) & 8238 & 8490  & 8363 & 8216 & 7929 & 8070 & 8227 & 8210 & 8216 & 8228 & 8228 & 8226 & 8228\\
%   RoBERTa (large) & 8175 & 8474 & 8322 & 8184 & 7843 & 8010 & 8180 & 8158 & 8166 & 8179 & 8179 & 8176 & 8179\\
% \hline
% \end{tabular}
% \end{table}


% \begin{sidewaystable}[h]
% \renewcommand\arraystretch{3}
% \setlength{\tabcolsep}{3pt}
% \caption{The results of algorithms performance for predicting both plurality and definiteness}
% \label{plurality and definiteness model performance}
% \centering
% \small
% \begin{tabular}{lccccccccccccccccccc}
% \hline
%   & \multicolumn{3}{c}{{\textsc{Single and Undefiniteness}}} & \multicolumn{3}{c}{{\textsc{Single and Definiteness}}} & \multicolumn{3}{c}{{\textsc{Plural and Definiteness}}} & \multicolumn{3}{c}{{\textsc{Plural and Undefiniteness}}} & \multicolumn{3}{c}{{\textsc{Macro avg}}} & \multicolumn{3}{c}{{\textsc{Weighted avg}}} &\\
%   & P & R & F & P & R & F & P & R & F & P & R & F & P & R & F & P & R & F & Acc.\\
% \hline
%   RF & 5358 & 8020 & 6424 & 6246 & 5705 & 5963 & 6741 & 2057 & 3152 & 6746 & 2003 & 3089 & 6273 & 4446 & 4657 & 6012 & 5755 & 5474 & 5755\\
%   LR & 5706 & 7373 & 6433 & 5999 & 6310 & 6150 & 5476 & 2466 & 3401 & 5856 & 2412 & 3417 & 5759 & 4640 & 4850 & 5811 & 5817 & 5616 & 5817\\
%   SVM & 5913 & 7468 & 6600 & 6324 & 6281 & 6302 & 5497 & 2963 & 3851 & 5329 & 3145 & 3956 & 5766 & 4964 & 5177 & 5943 & 5994 & 5857 & 5994\\
%   LSTM & 6839 & 7426 & 7120 & 6786 & 7271 & 7020 & 5198 & 4737 & 4957 & 5787 & 3604 & 4442 & 6152 & 5759 & 5885 & 6513 & 6580 & 6503 & 6580\\
%   BERT (base) & 7362 & 7799 & 7574 & 7359 & 7706 & 7528 & 5956 & 5312 & 5616 & 6271 & 4887 & 5493 & 6737 & 6426	& 6553 & 7072 & 7120 & 7079 & 7120\\
%   BERT (wwm, base) & 7387 & 7911 & 7640 & 7590 & 7533 & 7561 & 6223 & 5429 & 5799 & 5975 & 5423 & 5686 & 6794 & 6574 & 6672 & 7154 & 7186 & 7162 & 7186\\
%   BERT (multilingual, base) & 7482 & 7755 & 7616 & 7275 & 7839 & 7547 & 5744 & 5604 & 5673 & 6590 & 4633 & 5441 & 6773 & 6458 & 6569 & 7112 & 7146 & 7101 & 7146\\
%   RoBERTa (base) & 7620 & 7701 & 7660 & 7452 & 7850 & 7645 & 6100 & 5595 & 5836 & 6127 & 5423 & 5754 & 6825 & 6642 & 6724 & 7203 & 7236 & 7214 & 7236\\
%   RoBERTa (large) & 7424 & 7994 & 7698 & 7623 & 7761 & 7691 &	6351 & 5224 & 5733 & 6094 & 5226 & 5626 &	6873 & 6551	& 6687 & 7209 & 7255 & 7218 & 7255\\
% \hline
% \end{tabular}
% \end{sidewaystable}

% \begin{sidewaystable}[h]
% \renewcommand\arraystretch{3}
% \setlength{\tabcolsep}{3pt}
% \caption{Convergence of predicted results}
% \label{convergence of predicted results}
% \centering
% \small
% \begin{tabular}{lccccccccccccccccccc}
% \hline
%   & \multicolumn{3}{c}{{\textsc{Single and Undefiniteness}}} & \multicolumn{3}{c}{{\textsc{Single and Definiteness}}} & \multicolumn{3}{c}{{\textsc{Plural and Definiteness}}} & \multicolumn{3}{c}{{\textsc{Plural and Undefiniteness}}} & \multicolumn{3}{c}{{\textsc{Macro avg}}} & \multicolumn{3}{c}{{\textsc{Weighted avg}}} &\\
%   & P & R & F & P & R & F & P & R & F & P & R & F & P & R & F & P & R & F & Acc.\\
% \hline
%   RF & 5135 & 7972 & 6246 & 6003 & 5464 & 5721 & 5827 & 1442 & 2313 & 6402 & 1192 & 2010 & 5842 & 4017 & 4072 & 5696 & 5475 & 5084 & 5475\\
%   LR & 6015	& 7288 & 6590 & 6276 & 6485 & 6379 & 5294 & 3246 & 4024 & 5580 & 3223 & 4086 & 5791 & 5060 & 5270 & 5980 & 6036 & 5916 & 6036\\
%   SVM & 6033 & 7431 & 6659 & 6302 & 6320 & 6311 & 5161 & 3285 & 4014 & 5471 & 3195 & 4034 & 5742 & 5058 & 5255 & 5969 & 6032 & 5910 & 6032\\
%   LSTM & 6747 & 7174 & 6954	& 6240 & 7263 & 6713 & 5563 & 3721 & 4459 & 5777 & 3584 & 4424 & 6082 & 5436 & 5638 & 6315 & 6375 & 6276 & 6375\\
%   BERT (base) & 7404 & 7598 & 7500 & 7156 & 7553 & 7350 & 5771 & 5178 & 5459 & 5916 & 5012 & 5426 & 6562 & 6335 & 6434 & 6949 & 6991 & 6961 & 6991\\
%   BERT (wwm, base) & 7383 & 7813 & 7592 & 7243 & 7312 & 7277 & 6124 & 5230 & 5642 & 5853 & 5338 & 5584 & 6651 & 6423 & 6524	& 7003 & 7040 & 7014 & 7040\\
%   BERT (multilingual, base) & 7145 & 7776 & 7448 & 7182 & 7126 & 7154 & 5738 & 4562 & 5083 & 5612 & 5138 & 5365 & 6419 & 6151	& 6262 & 6811 & 6859 & 6821 & 6859\\
%   RoBERTa (base) & 7293 & 7907 & 7588 & 7342 & 7410 & 7376 & 6101 & 5009 & 5501 & 6094 & 5229 & 5629 & 6708 & 6389 & 6523 & 7029 & 7074 & 7036 & 7074\\
%   RoBERTa (large) & 7234 & 7975 & 7587 & 7233 & 7265 & 7249 & 5996 & 4846 & 5360 & 6379 & 5256 & 5763 & 6711 & 6336	& 6490 & 6990 & 7035 & 6992	& 7035\\
% \hline
% \end{tabular}
% \end{sidewaystable}

\begin{table}[H]
\caption{The results of algorithms performance for plurality}
\label{plurality model performance}
\centering
\small
\begin{tabular}{lccccccc}
\hline
  & \multicolumn{3}{c}{{\textsc{Macro avg}}} & \multicolumn{3}{c}{{\textsc{Weighted avg}}} &\\
  & P & R & F & P & R & F & Acc.\\
  \hline
  RF & 81.08 & 58.19 & 58.53 & 80.26 & 79.69 & 74.19 & 79.69\\
  LR & 76.08 & 67.39 & 69.79 & 80.11 & 81.58 & 79.77 & 81.58\\
  SVM & 75.56 & 67.37 & 69.69 & 79.88 & 81.40 & 79.65 & 81.40\\
  LSTM & 79.31 & 70.94 & 73.59 & 82.49 & 83.50 & 82.14 & 83.50\\
  BERT (base) & 80.88 & 77.96 & 79.24 & 85.23 & 85.73 & 85.37 & 85.73\\
  BERT (wwm,base) & 80.94 & 78.34 & 79.50 & 85.38 & 85.83 & 85.52 & 85.83\\
  BERT (multilingual,base) & 80.07 & 76.96 & 78.30 & 84.58 & 85.15 & 84.74 & 85.15\\
  RoBERTa (base) & 81.21 & 77.53 & 79.09 & 85.22 & 85.79 & 85.35 & 85.79\\
  RoBERTa (large) & 81.72 & 77.37 & 79.17 & 85.38 & 85.98 & 85.46 & 85.98\\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\caption{The results of algorithms performance for definiteness}
\label{definiteness model performance}
\centering
\small
\begin{tabular}{lccccccc}
\hline
  & \multicolumn{3}{c}{{\textsc{Macro avg}}} & \multicolumn{3}{c}{{\textsc{Weighted avg}}} &\\
  & P & R & F & P & R & F & Acc.\\
  \hline
  RF & 68.63 & 67.24 & 67.10 & 68.51 & 68.09 & 67.47 & 68.09\\
  LR & 71.73 & 71.53 & 71.58 & 71.78 & 71.82 & 71.75 & 71.82\\
  SVM & 71.34 & 71.04 & 71.10 & 71.37 & 71.40 & 71.29 & 71.40\\
  LSTM & 76.78 & 76.88 & 76.80 & 76.95 & 76.84 & 76.87 & 76.84\\
  BERT (base) & 81.60 & 81.66 & 81.63 & 81.71 & 81.69 & 81.69 & 81.69\\
  BERT (wwm, base) & 81.95 & 81.82 & 81.87 & 81.98 & 81.98 & 81.97 & 81.98\\
  BERT (multilingual, base) & 80.70 & 80.41 & 80.50 & 80.68 & 80.66 & 80.62 & 80.66\\
  RoBERTa (base) & 82.27 & 82.10 & 82.16 & 82.28 & 82.28 & 82.26 & 82.28\\
  RoBERTa (large) & 81.80 & 81.58 & 81.66 & 81.79 & 81.79 & 81.76 & 81.79\\
\hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{The results of algorithms performance for predicting both plurality and definiteness}
\label{plurality and definiteness model performance}
\centering
\small
\begin{tabular}{lccccccc}
\hline
  & \multicolumn{3}{c}{{\textsc{Macro avg}}} & \multicolumn{3}{c}{{\textsc{Weighted avg}}} &\\
  & P & R & F & P & R & F & Acc.\\
\hline
  RF & 62.73 & 44.46 & 46.57 & 60.12 & 57.55 & 54.74 & 57.55\\
  LR & 57.59 & 46.40 & 48.50 & 58.11 & 58.17 & 56.16 & 58.17\\
  SVM & 57.66 & 49.64 & 51.77 & 59.43 & 59.94 & 58.57 & 59.94\\
  LSTM & 61.52 & 57.59 & 58.85 & 65.13 & 65.80 & 65.03 & 65.80\\
  BERT (base) & 67.37 & 64.26	& 65.53 & 70.72 & 71.20 & 70.79 & 71.20\\
  BERT (wwm, base) & 67.94 & 65.74 & 66.72 & 71.54 & 71.86 & 71.62 & 71.86\\
  BERT (multilingual, base) & 67.73 & 64.58 & 65.69 & 71.12 & 71.46 & 71.01 & 71.46\\
  RoBERTa (base) & 68.25 & 66.42 & 67.24 & 72.03 & 72.36 & 72.14 & 72.36\\
  RoBERTa (large) & 68.73 & 65.51	& 66.87 & 72.09 & 72.55 & 72.18 & 72.55\\
\hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Convergence of predicted results}
\label{convergence of predicted results}
\centering
\small
\begin{tabular}{lccccccc}
\hline
  &\multicolumn{3}{c}{{\textsc{Macro avg}}} & \multicolumn{3}{c}{{\textsc{Weighted avg}}} &\\
  &P & R & F & P & R & F & Acc.\\
\hline
  RF & 58.42 & 40.17 & 40.72 & 56.96 & 54.75 & 50.84 & 54.75\\
  LR & 57.91 & 50.60 & 52.70 & 59.80 & 60.36 & 59.16 & 60.36\\
  SVM & 57.42 & 50.58 & 52.55 & 59.69 & 60.32 & 59.10 & 60.32\\
  LSTM & 60.82 & 54.36 & 56.38 & 63.15 & 63.75 & 62.76 & 63.75\\
  BERT (base) & 65.62 & 63.35 & 64.34 & 69.49 & 69.91 & 69.61 & 69.91\\
  BERT (wwm, base) & 66.51 & 64.23 & 65.24 & 70.03 & 70.40 & 70.14 & 70.40\\
  BERT (multilingual, base) & 64.19 & 61.51 & 62.62 & 68.11 & 68.59 & 68.21 & 68.59\\
  RoBERTa (base) & 67.08 & 63.89 & 65.23 & 70.29 & 70.74 & 70.36 & 70.74\\
  RoBERTa (large) & 67.11 & 63.36	& 64.90 & 69.90 & 70.35 & 69.92 & 70.35\\
\hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Bert Accuracy Result with Different Context Length}
\label{Bert Predict Result with Different Context Length}
\centering
\small
\begin{tabular}{lccccc}
\hline
  &n=0 & n=1 & n=2 & n=3 & n=4\\
\hline
  Plurality & 85.37 & 84.77 & 84.95 & 84.09 & 84.16\\
  Definiteness & 81.69 & 79.81 & 79.69 & 79.46 & 79.54\\
\hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Model prediction results for explicit and implicit expressions of plurality}
\label{Bert Predict Result with Different Context Length}
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
&         & \multicolumn{3}{c}{Macro avg} & \multicolumn{3}{c}{Weighted avg} &        \\ 
\cmidrule(l){3-5} 
\cmidrule(l){6-8} 
&         & P        & R        & F       & P         & R         & F        & Acc.   \\
\midrule
\multirow{2}{*}{RF}  & implict & 59.05   & 82.63   & 60.01  & 94.86    & 80.74    & 85.83   & 80.74 \\
\cmidrule(l){2-2} 
& explict & 52.92   & 66.56   & 48.59  & 94.52    & 71.82    & 80.53   & 71.82 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{LR}  & implict & 68.25   & 76.99   & 70.80  & 87.24    & 82.51    & 84.17   & 82.51 \\
\cmidrule(l){2-2} 
& explict & 62.01   & 69.45   & 62.99  & 83.04    & 74.61    & 77.52   & 74.61 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{SVM}  & implict & 68.08   & 76.16   & 70.49  & 86.69    & 82.19    & 83.80   & 82.19 \\
\cmidrule(l){2-2} 
& explict & 63.01   & 71.06   & 64.18  & 83.74    & 75.43    & 78.25   & 75.43 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{LSTM} & implict & 69.52   & 78.31   & 72.19  & 87.61    & 83.23    & 84.75   & 83.23 \\
\cmidrule(l){2-2} 
& explict & 79.26   & 84.27   & 81.15  & 87.41    & 85.54    & 86.11   & 85.54 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{BERT(base)} & implict & 77.13   & 80.29   & 78.50  & 86.61    & 85.61    & 86.01   & 85.61 \\
\cmidrule(l){2-2} 
& explict & 82.78   & 84.15   & 83.41  & 86.95    & 86.61    & 86.74   & 86.61 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{BERT(wwm, base)} & implict & 77.25   & 80.04   & 78.48  & 86.38    & 85.51    & 85.86   & 85.51 \\
\cmidrule(l){2-2} 
& explict & 84.86   & 86.18   & 85.47  & 88.53    & 88.25    & 88.36   & 88.25 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{BERT (multilingual, base)} & implict & 76.07   & 79.11   & 77.39  & 85.90    & 84.87    & 85.28   & 84.87 \\
\cmidrule(l){2-2} 
& explict & 82.40   & 85.76   & 83.81  & 88.23    & 87.26    & 87.58   & 87.26 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{RoBERTa (base)} & implict & 76.60   & 80.61   & 78.28  & 86.98    & 85.65    & 86.16   & 85.65 \\
\cmidrule(l){2-2} 
& explict & 82.95   & 84.53   & 83.67  & 87.25    & 86.85    & 87.01   & 86.85 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{RoBERTa (large)} & implict & 76.34   & 80.97   & 78.23  & 87.30    & 85.75    & 86.33   & 85.75 \\
\cmidrule(l){2-2} 
& explict & 83.44   & 85.90   & 84.53  & 88.30    & 87.67    & 87.89   & 87.67 \\ 
\midrule
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Model prediction results for explicit and implicit expressions of definiteness}
\label{Bert Predict Result with Different Context Length}
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
&         & \multicolumn{3}{c}{Macro avg} & \multicolumn{3}{c}{Weighted avg} &        \\ 
\cmidrule(l){3-5} 
\cmidrule(l){6-8} 
&         & P        & R        & F       & P         & R         & F        & Acc.   \\
\midrule
\multirow{2}{*}{RF}  & implict & 66.91 & 68.37 & 67.11 & 71.09 & 68.86 & 69.50 & 68.86 \\
\cmidrule(l){2-2} 
& explict & 68.05 & 67.33 & 65.02 & 69.82 & 65.11 & 64.76 & 65.11 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{LR}  & implict & 71.16 & 71.24 & 71.20 & 71.93 & 71.87 & 71.90 & 71.87 \\
\cmidrule(l){2-2} 
& explict & 72.45 & 71.12 & 71.00 & 72.31 & 71.62 & 71.18 & 71.62 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{SVM}  & implict & 70.70 & 70.92 & 70.79 & 71.76 & 71.57 & 71.65 & 71.57 \\
\cmidrule(l){2-2} 
& explict & 71.62 & 70.32 & 70.13 & 71.49 & 70.73 & 70.28 & 70.73 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{LSTM} & implict & 75.21 & 75.03 & 75.11 & 75.49 & 75.55 & 75.51 & 75.55 \\
\cmidrule(l){2-2} 
& explict & 79.30 & 81.32 & 80.05  & 82.86 & 81.83 & 82.13   & 81.83 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{BERT(base)} & implict & 80.64 & 80.52 & 80.58  & 80.93 & 80.96 & 80.94 & 80.96 \\
\cmidrule(l){2-2} 
& explict & 83.12 & 83.63 & 83.36  & 84.65 & 84.50 & 84.56   & 84.50 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{BERT(wwm, base)} & implict & 80.44 & 80.81 &  80.60  & 81.29 & 81.13 & 81.18   & 81.13 \\
\cmidrule(l){2-2} 
& explict & 84.21 & 84.38 & 84.29  & 85.33 & 85.29 & 85.31    & 85.29 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{BERT (multilingual, base)} & implict & 78.78 & 79.30 & 78.99  & 79.89 & 79.61 & 79.70   & 79.61 \\
\cmidrule(l){2-2} 
& explict & 84.42 & 83.59 & 83.94  & 84.67 & 84.73 & 84.64   & 84.73 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{RoBERTa (base)} & implict & 80.87 & 81.18 & 81.00 & 81.63 & 81.50 & 81.55 & 81.50 \\
\cmidrule(l){2-2} 
& explict & 84.87 & 84.19 & 84.49 & 85.22 & 85.29 & 85.22 & 85.29 \\
\cmidrule(l){1-2} 
\multirow{2}{*}{RoBERTa (large)} & implict & 79.92 & 80.57 & 80.17 & 81.14 & 80.79 & 80.89 & 80.79 \\
\cmidrule(l){2-2} 
& explict & 84.21 & 85.00 & 84.56 & 85.90 & 85.67 & 85.75 & 85.67 \\ 
\midrule
\end{tabular}
\end{table}

\end{document}

